Parameterized Intractability of Even Set and Shortest Vector Problem from Gap-ETH

The $k$-Even Set problem is a parameterized variant of the Minimum Distance Problem of linear codes over $\mathbb F_2$, which can be stated as follows: given a generator matrix $\mathbf A$ and an integer $k$, determine whether the code generated by $\mathbf A$ has distance at most $k$. Here, $k$ is the parameter of the problem. The question of whether $k$-Even Set is fixed parameter tractable (FPT) has been repeatedly raised in literature and has earned its place in Downey and Fellows' book (2013) as one of the "most infamous" open problems in the field of Parameterized Complexity. In this work, we show that $k$-Even Set does not admit FPT algorithms under the (randomized) Gap Exponential Time Hypothesis (Gap-ETH) [Dinur'16, Manurangsi-Raghavendra'16]. In fact, our result rules out not only exact FPT algorithms, but also any constant factor FPT approximation algorithms for the problem. Furthermore, our result holds even under the following weaker assumption, which is also known as the Parameterized Inapproximability Hypothesis (PIH) [Lokshtanov et al.'17]: no (randomized) FPT algorithm can distinguish a satisfiable 2CSP instance from one which is only $0.99$-satisfiable (where the parameter is the number of variables). We also consider the parameterized $k$-Shortest Vector Problem (SVP), in which we are given a lattice whose basis vectors are integral and an integer $k$, and the goal is to determine whether the norm of the shortest vector (in the $\ell_p$ norm for some fixed $p$) is at most $k$. Similar to $k$-Even Set, this problem is also a long-standing open problem in the field of Parameterized Complexity. We show that, for any $p > 1$, $k$-SVP is hard to approximate (in FPT time) to some constant factor, assuming PIH. Furthermore, for the case of $p = 2$, the inapproximability factor can be amplified to any constant.

==> csp-to-vectorsum-back-up.tex <==
\section{Reducing $\csp$ to $\gapvec$} \label{sec:main-red}

\begin{lemma}						
For any constant $\varepsilon > 0$ and any positive integer $d \in \mathbb{N}$, there exists an FPT reduction from $\csp_{\varepsilon}(d)$ to $\gapvec_{\gamma}$ where $\gamma = 1 + \frac{\varepsilon}{3(d + 1)}$.
\end{lemma}

\begin{proof}
Let $\Gamma = (G = (V, E), \Sigma, \{C_{uv}\}_{(u, v) \in E})$ is the input for $\csp_{\varepsilon}(d)$. We produce an instance $(\bA, \by, k)$ of $\gapvec_{\gamma}$ as follows. Let $n = |V| + |E| + 2 |E| |\Sigma|$ and $m = |V| + \sum_{(u, v) \in E} |C_{uv}|$; our matrix $\bA$ will be of dimension $(n \times m)$. For convenient, let us label the first $|V|$ rows of $\bA$ by the vertices $u \in V$, the next $|E|$ rows by the edges $e \in E$, and the last $2 |E| |\Sigma|$ rows by a tuple $(e, \sigma, b) \in E \times \Sigma \times \{0, 1\}$. Furthermore, we label the first $|V|$ rows of $\bA$ by $(u, \sigma_u)$ where $u \in V$ and $\sigma_u \in \Sigma$, and the rest of the rows by $(e, \sigma_0, \sigma_1)$ where $e \in E$ and $(\sigma_0, \sigma_1) \in C_e$. The entries of our matrix $\bA \in \F^{n \times m}$ can now be defined as follows.
\begin{itemize}
\item For each column of the form $(u, \sigma_u)$, let the following entries be one: 
\begin{itemize}
\item $\bA_{u, (u, \sigma_u)}$.
\item $\bA_{((u, v), \sigma_u, 0), (u, \sigma_u)}$ for every $v \in V$ such that $(u, v) \in E$.
\item $\bA_{((v, u), \sigma_u, 1), (u, \sigma_u)}$ for every $v \in V$ such that $(v, u) \in E$.
\end{itemize}
The rest of the entries are set to zero.
\item For each column of the form $(e, \sigma_0, \sigma_1)$, we define the entries as follows.
\begin{itemize}
\item Let $\bA_{e, (e, \sigma_0, \sigma_1)} = 1$.
\item For every $\sigma \in \Sigma$ and $b \in \{0, 1\}$, let
\begin{align*}
\bA_{(e, \sigma, b), (e, \sigma_1, \sigma_2)} = \ind[\sigma \ne \sigma_b].
\end{align*}
\end{itemize}
The rest of the entries are set to zeros.
\end{itemize}
Finally, we set $\by = \vone_n$ be the all ones vector and $k = |V| + |E|$.

{\bf Parameter Dependency.} The new parameter $k$ is simply $|V| + |E|$. Since we assume that the degree of every vertex is bounded by some constant $d$, we have $|V| + |E| = O(|V|)$.

Before we move on to prove the completeness and soundness of the reduction, let us state an observation that will be useful in the analysis:
\begin{observation}
For any $\bx \in \F^{m}$, the following properties hold.
\begin{itemize}
\item For every row of the form $u \in V$, we have 
\begin{align}
(\bA\bx)_{u} = \sum_{\sigma_u \in \Sigma} \bx_{(u, \sigma)}.
\label{eq:row-1}
\end{align}
\item For every row of the form $e \in E$, we have
\begin{align}
(\bA\bx)_e = \sum_{(\sigma_0, \sigma_1) \in C_e} \bx_{(e, \sigma_0, \sigma_1)}.
\label{eq:row-2}
\end{align}
\item For every row of the form $(e = (u_0, u_1), \sigma, b)$, we have
\begin{align}
(\bA\bx)_{(e, \sigma, b)} = \bx_{(u_b, \sigma)} + \sum_{(\sigma_0, \sigma_1) \in C_e \atop \sigma_b \ne \sigma} \bx_{(e, \sigma_0, \sigma_1)}.
\label{eq:row-3}
\end{align}
\end{itemize}
\end{observation}
Note that the above observation follows trivially from our definition of $\bA$.

{\bf Completeness.} Suppose that $\val(\Gamma) = 1$. That is, ther exists an assignment $\psi: V \to \Sigma$ that satisfies all the edges. We define the vector $\bx \in \F^m$ as follows.
\begin{itemize}
\item For each $(u, \sigma)$, let $\bx_{(u, \sigma)} = \ind[\psi(u) = \sigma]$
\item For each $(e = (u, v), \sigma_0, \sigma_1)$, let $\bx_{(e, \sigma_0, \sigma_1)} = \ind[(\psi(u) = \sigma_0) \wedge (\psi(v) = \sigma_1)]$.
\end{itemize}
We claim that $\bA\bx = \by$. To see that this is the case, consider the following three cases of rows.
\begin{itemize}
\item For each row of the form $u \in V$, we have
\begin{align*}
(\bA\bx)_{u} \overset{(\ref{eq:row-1})}{=} \sum_{\sigma \in \Sigma} \bx_{(u, \sigma)} = \sum_{\sigma \in \Sigma} \ind[\psi(u) = \sigma] = 1.
\end{align*}
\item For each row of the form $e = (u, v) \in E$, we have 
\begin{align*}
(\bA\bx)_e \overset{(\ref{eq:row-2})}{=} \sum_{(\sigma_0, \sigma_1) \in C_e} \bx_{(e, \sigma_0, \sigma_1)} = \sum_{(\sigma_0, \sigma_1) \in C_e} \ind[(\psi(u) = \sigma_0) \wedge (\psi(v) = \sigma_1)] = 1.
\end{align*}
Note that, in the last equality, we use the fact that the edge $e$ is satisfied (i.e. $(\psi(u), \psi(v)) \in C_e$).
\item For each row $(e = (u_0, u_1), \sigma, b) \in E \times \Sigma \times \{0, 1\}$, we have 
\begin{align*}
(\bA\bx)_{(e, \sigma, b)} \overset{(\ref{eq:row-3})}{=} \bx_{(u_b, \sigma)} + \sum_{(\sigma_0, \sigma_1) \in C_e \atop \sigma_b \ne \sigma} \bx_{(e, \sigma_0, \sigma_1)} = \ind[\psi(u_b) = \sigma] + \ind[\psi(u_b) \ne \sigma] = 1,
\end{align*}
where the second equality uses the fact that exactly one of $\bx_{(e, \sigma_0, \sigma_1)}$ is not zero among $(\sigma_0, \sigma_1) \in C_e$, which is $\bx_{(e, \psi(u_0), \psi(u_1))}$.
\end{itemize}

Hence, $\bA\bx$ is indeed equal to $\by = \vone_n$. Finally, observe that $\|x\|_H = |V| + |E|$ as desired.

{\bf Soundness.} We will prove this by contrapositive. Suppose that the constructed instance $(\bA, \by, k)$ is not a NO instance of $\gapvec_\gamma$, i.e., for some $x \in \cB^{m}_H(\bzero, \gamma k)$, $\bA\bx = \by$. We will show that $\Gamma$ is not a NO instance of $\csp_{\varepsilon}(d)$, i.e., that $\val(\Gamma) \geqs 1 - \varepsilon$.

First, for each vertex $u \in V$, let $S_u = \{\sigma \in \Sigma \mid \bx_{(u, \sigma)} = 1\}$ and, for each $e \in E$, let $T_e = \{(\sigma_0, \sigma_1) \in C_e \mid \bx_{(e, \sigma_0, \sigma_1)} = 1\}$. From (\ref{eq:row-1}) and from $(\bA\bx)_u = \by_u = 1$, we can conclude that $|S_u| \geqs 1$ for all $u \in V$. Similarly, from (\ref{eq:row-2}) and from $(\bA\bx)_e = \by_e = 1$, we have $|T_e| \geqs 1$ for all $e \in E$.

Let $V_{\uni}$ denote the set of $u \in V$ such that $|S_u| = 1$. For each $u \in V_{\uni}$, let $\sigma_u$ be the only element of $S_u$. We define an assignment $\psi: V \to \Sigma$ of $\Gamma$ by setting $\psi(u) = \sigma_u$ for all $u \in V_{\uni}$ and $\psi(u)$ arbritarity otherwise. We will show that $\val(\psi) \geqs 1 - \varepsilon$, which indeed implies $\val(\Gamma) \geqs 1 - \varepsilon$.

To do so, let $E_{\uni}$ denote the set of $e \in E$ such that $|T_e| = 1$. Furthermore, let $E^*$ denote the set of $e = (u, v) \in E_{\uni}$ such that both $u, v$ are in $V_{\uni}$.

Notice that
\begin{align*}
(\gamma - 1) k &\geqs \|\bx\|_H - k \\ 
&= \sum_{u \in V} |S_u| + \sum_{e \in E} |T_e| - k \\
&= \sum_{u \in V} (|S_u| - 1) + \sum_{e \in E} (T_e - 1) \\
&\geqs \sum_{u \in V \setminus V_{\uni}} (|S_u| - 1) + \sum_{e \in E \setminus E_{\uni}} (T_e - 1) \\
&\geqs \sum_{u \in V \setminus V_{\uni}} 1 + \sum_{e \in E \setminus E_{\uni}} 1 \\
&\geqs |V \setminus V_{\uni}| + |E \setminus E_{\uni}|,
\end{align*}
which implies that $|V_{\uni}| \geqs |V| - (\gamma - 1)k$ and $|E_{\uni}| \geqs |E| - (\gamma - 1)k$. Additionally, note that the set $E_{\uni} \setminus E^*$ contains only $(u, v) \in E$ such that $u \in (V \setminus V_{\uni})$ or $v \in (V \setminus V_{\uni})$. Since $|V \setminus V_{\uni}| \leqs (\gamma - 1)k$ and every vertex in $G$ has degree at most $d$, we have $|E_{\uni} \setminus E^*| \leqs d(\gamma - 1)k$. As a result, we have $|E^*| \geqs |E| - (d + 1)(\gamma - 1)k$, which, from our choice of $\gamma$, is at least $|E| - \frac{\varepsilon k}{3} \geqs (1 - \varepsilon)|E|$. Note that the last inequality follows from $|V| \leqs 2|E|$, which can be assumed without loss of generality.

Since $|E^*| \geqs (1 - \varepsilon)|E|$, to show that $\val(\psi) \geqs 1 - \varepsilon$, it suffices to show that $\psi$ satisfies every edge $e \in E^*$. To see that this is the case, let $e = (u, v)$ be any edge in $E^*$. Let $(\sigma^*_0, \sigma^*_1)$ be the only element of $T_e$. Observe that, from (\ref{eq:row-3}) with $\sigma = \sigma_u$ and $b = 0$ and from $(\bA\bx)_{e, \sigma, b} = \by_{e, \sigma, b} = 1$, we can conclude that $\sigma^*_0 = \sigma_u$. Similarly, we can conclude that $\sigma^*_1 = \sigma_v$. As a result, $(\sigma_u, \sigma_v)$ must be in $C_e$, meaning that $\psi$ satisfies the edge $e$, which completes our proof.
\end{proof}

==> svp.tex <==
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bW}{\mathbf{W}}


\section{Parameterized Intractability of Shortest Vector Problem}\label{sec:svp}

We begin by stating the intractability of $\snvp_{p,\eta}$, which is the main result of this section:

\begin{theorem}[FPT Inapproximability of $\svp$]\label{thm:SVPmain}
Assuming PIH, for any $\gamma \geqs 1$, any $p > 1$, there is no randomized FPT algorithm for $\svp_{p,\gamma}$.
\end{theorem}

The proof of Theorem~\ref{thm:SVPmain} goes through the following FPT inapproximability of $\snvp_{p,\eta}$. 

\begin{theorem}[FPT Inapproximability of $\snvp$]\label{thm:CVPmain}
Assuming PIH, for any $\gamma, p \geqs 1$, there is no FPT algorithm which on input $(\bB, \by, t)$ where $\bB \in \Z^{n \times q}, \by \in \Z^n$ and $t \in \N$, can distinguish between
\begin{itemize}
	\item (YES) there exists $\bx \in \Z^q$ such that $\|\bB \bx - \by \|^p_p \leqs t$.
	\item (NO) for all choices of $\bx \in \Z^q$, we have $\|\bB \bx - \by \|^p_p > \gamma \cdot t$
\end{itemize} 
\end{theorem}

The above theorem follows from the following reduction from $\csp_\epsilon$ to $\snvp_{p,\eta}$.

\begin{lemma} \label{lem:csp-to-snvp}		
	For any $\eta, p \geqs 1$ and $\epsilon > 0$, there is an FPT reduction from $\csp_\epsilon$ instance $\Gamma$ to $\snvp_{p,\eta}$ instance $(\bB,\by,t)$. Moreover, this reduction satisfies the following stronger properties:
	\begin{itemize}
		%\item The matrix $\bB \in \Z^{n \times q}$ and the vector $\by \in \Z^n$ are of dimensions polynomial in the size of $\Gamma$.
		\item If $\Gamma$ is a YES instance, then there exists $\bx \in \Z^{q}$ such that $\bB \bx - \by$ is a $\{0,1\}$-vector of Hamming weight at most $t$.
		\item If $\Gamma$ is a NO instance, then for all choices of $\bx \in \Z^q$ and $w \in \Z \setminus \{0\}$, we have $\|\bB \bx - w\cdot\by\|_0 > \eta\cdot t$.
	\end{itemize}
\end{lemma}

The proof of the above Lemma is identical to FPT reduction of $\csp$ to $\sncp$, we defer it to Appendix~\ref{sec:csp-to-snvp}. Note that the reduction has stronger guarantees than a usual reduction from $\csp_\epsilon$ to $\snvp_{p,\eta}$ in both the YES and NO cases. In the YES case, the witness ot the $\snvp$ instance is a $\{0,1\}$-vector. Furthermore, in the NO case of the above lemma, the lower bound guarantee is in terms of the Hamming norm. These properties are used crucially in the analysis for  the reduction from $\snvp_{p,\eta}$ to $\svp_{p,\gamma}$. The proof of Theorem \ref{thm:SVPmain} also requires the following definition of annoying vectors.

\begin{definition}[Annoying Vectors]				\label{def:annoying-vectors}
	Given $\bA \in \Z^{u \times v}$ and a parameter $l \in \mathbb{N}$, we say a vector $\bz := \bA \bx$ (for some $\bx \in \Z^v$) is an \emph{Annoying Vector}, if it violates all of the following conditions:
	\begin{itemize}
		\item[1.] The Hamming weight of $\bz$ at least $l$.
		\item[2.] All coordinates of $\bz$ are even, and its Hamming weight is at least $l/2^p$.
		\item[3.] All coordinates of $\bz$ are even, and it has at least one coordinate of magnitude at least $l^{10l}$. 
	\end{itemize}
\end{definition}

As shown later in Section \ref{sec:svp-gap-amp}, lattices without annoying vectors are ``well behaved'' with respect to tensor products of lattices. This notion will be useful later, when the lattice tensor product is used to amplify the gap to any constant. 

The second step is a randomized FPT reduction from $\snvp_{p,\eta}$ to $\svp_{p,\gamma}$, as stated by the following lemma:

\begin{lemma}				\label{lem:snvp-to-svp}
	Fix $p > 1$, and let $\eta \geqs 1$ be such that $\frac12 + \frac{1}{2^p} + \frac{(2^p + 1)}{\eta} < 1$. Let $(\bB,\by,t)$ be a $\snvp_{p,\eta}$ instance, as given by Lemma \ref{lem:csp-to-snvp}. Then, for some constant $\gamma_p > 1$, there is a randomized FPT reduction from $\snvp_{p,\eta}$ instance $(\bB,\by,t)$ to $\svp_{p,\gamma}$ instance $(\bB_{\rm svp},\gamma^{-1}_pl)$ with $l = \eta \cdot t$ such that
	\begin{itemize}
		\item The matrix $\bB_{\rm svp}$ is of dimensions $(n + m + h + 1) \times (q + m + h + 2)$, where $m = l^{O(l)}\cdot{\rm poly}(n,q)$ and $h = {\rm poly}(l,n,q)$.
		\item If $(\bB,\by,t)$ is a YES instance, then w.p. $0.8$, there exists $\bx \in \Z^{q + m + h + 2}$ such that $\|\bB_{\rm svp}\bx\|^p_p \leqs \gamma^{-1}_p l$.
		\item If $(\bB,\by,t)$ is a NO instance, then w.p. $0.9$, for all choices of $\bx \in \Z^{q + m + h + 2}$, the vector $\bB_{\rm svp}\bx$ is not annoying. In particular, for every choice of $\bx \in \Z^{q + m + h + 2}$ we have $\|\bB_{\rm svp}\bx\|^p_p \geqs l$.
	\end{itemize}
\end{lemma}

Combining the above lemma with Lemma~\ref{lem:csp-to-snvp}, followed by gap amplification (Section~\ref{sec:svp-gap-amp}) gives us Theorem \ref{thm:SVPmain}. The reduction in the above lemma is nearly identical to the one from \cite{Khot05}. We devote the rest of this section to describing this reduction and proving Lemma \ref{lem:snvp-to-svp}. 

The rest of this section is organized as follows. In Section \ref{sec:bch-lattic}, we define the BCH lattice, which is the key gadget used in the reduction. Using the BCH lattice and the $\snvp_{p, \eta}$ instance, we construct the intermediate lattice in Section \ref{sec:int-lattice}. The intermediate lattice serves to blow up the number of potential witnesses for the YES case (aka the good vectors), while controlling the number of potential annoying vectors for the NO case. In particular, this step ensures that the number of good vectors (Lemma \ref{lem:good-vectors}) far outnumber the number of annoying vectors (Lemma \ref{lem:annoying-vectors}). Finally, in Section \ref{sec:final-lattice} we compose the intermediate lattice with an random homogeneous constraint (sampled from an appropriate distribution), to give the final $\svp_{p,\gamma}$ instance. The additional random constraint is used to annihilate potential annoying vectors in the NO case, while retaining at least one potential witness in the YES case (Lemma \ref{lem:svp-lattice}).

{\noindent{\bf Setting}: For the rest of the section, we will fix $(\bB,\by,t)$ to be a $\snvp_{p,\eta}$ instance (as given by Lemma \ref{lem:csp-to-snvp}) and we set $l := \eta \cdot t$.}

\subsection{The BCH Lattice gadget}				\label{sec:bch-lattic}

We begin by defining the BCH lattices which is the key gadget used in the reduction. Given parameters $l,m \in \mathbb{N}$ where $m$ is a power of $2$, the BCH lattice is defined by the generator $\bB_{\rm BCH}$ defined as
\begin{align*}
	\bB_{\rm BCH} =
	\begin{bmatrix}
		{\rm Id}_{m} &  \mathbf{0}_{m \times h} \\
		Q\cdot\mathbf{P}_{\rm BCH} & 2Q\cdot{\rm Id}_{h}
	\end{bmatrix}
	\in \mathbb{Z}^{(m + h) \times (m + h)}.
\end{align*}
\noindent where $\mathbf{P}_{\rm BCH} \in \{0,1\}^{h \times m}$ is the parity check matrix of a $[m,m-h,l]_2$-BCH code (i.e., $h$ is the codimension of the code whose parity check matrix is ${\bf P}_{\rm BCH}$), and $Q = l^{10l}$. By our choice of parameters it follows that $h \leqs \frac{l}{2}\log m$ (see Theorem \ref{thm:bch}). The following lemma summarizes the key properties of BCH lattices, as defined above.

\begin{lemma}				\label{lem:bch-lattice}
	Let $\mathbf{B}_{\rm BCH} \in \mathbb{Z}^{(m + h) \times ( m + h)}$ be the BCH lattice constructed as above. Let $ r = \Big(\frac12 + \frac{1}{2^p} + \frac{1}{\eta}\Big)\eta t$. Then there exists a randomized polynomial time algorithm, which with probability at least $0.99$, returns vector $\mathbf{s} \in \mathbb{Z}^{m+h}$ such that the following holds. There exists at least $\frac{1}{100}2^{-h}{m \choose r}$ distinct coefficient vectors $\mathbf{z} \in \mathbb{Z}^{m + h}$ such that the vector $\big(\mathbf{B}_{\rm BCH} \mathbf{z} - \mathbf{s}\big)$ is a $\{0,1\}$-vector of Hamming weight exactly $r$.
\end{lemma}

We skip the proof of the above lemma, since it is identical to proof of Lemma 4.3 in \cite{Khot05}. Note that this is in fact even weaker than Khot's lemma, since we do not impose a bound on $\|\mathbf{z}\|_p$.

\subsection{The Intermediate Lattice}			\label{sec:int-lattice}

We now define the intermediate lattice. Let $(\bB,\by,t)$ be an instance of $\snvp_{p,\eta}$, where $\bB \in \Z^{n \times q}$. The intermediate lattice $\bB_{\rm int}$ is constructed as follows. Let $l = \eta t$. Let $m$ be the smallest power of 2 such that $m \geqs \max\{2^{10p+10}n, (100l)^{100\eta l}\}$, and let $\bB_{\rm BCH}$ be constructed as above. Then 
\begin{align*}
	\bB_{\rm int} =
	\begin{bmatrix}
		2\bB &  \mathbf{0}_{ n \times  (m+h)} &  2\by  \\
		\mathbf{0}_{(m + h) \times q} &  \bB_{\rm BCH} &  \bs
	\end{bmatrix}
	\in \Z^{(n + m + h) \times (q + m + h + 1)}.
\end{align*}
where $\mathbf{s} \in \Z^{m + h}$ is the vector given by Lemma \ref{lem:bch-lattice}. The following lemmas bound the good and annoying vectors in the YES and NO cases respectively.

\begin{lemma}				\label{lem:good-vectors}
   Let $(\mathbf{B},\mathbf{y},t)$ be a YES instance, and let $\mathbf{B}_{\rm int}$ be the corresponding intermediate lattice. Then, with probability at least $0.99$, there exists at least distinct ${m^{r}}\Big({100 m^{l/2}l^{l}}\Big)^{-1}$ vectors $\mathbf{x} \in \mathbb{Z}^{q + m + h + 1}$ such that $\mathbf{B}_{\rm int}\mathbf{x}$ are distinct $\{0,1,2\}$-vectors with $\ell_p$ norm at most $(2^p t + r)^{1/p}$.
\end{lemma}
\begin{proof}
	Let $\tbx \in \mathbb{Z}^{q}$ be vector such that ${\bf B}\tbx - {\bf y}$ is a $\{0,1\}$-vector of Hamming weight at most $t$. From Lemma \ref{lem:bch-lattice}, there exists at least $2^{-h}{m \choose r}/100$ distinct vectors ${\bf z} \in \mathbb{Z}^{m + h}$ such that ${\bf B}_{\rm BCH}{\bf z} - {\bf s}$ is a $\{0,1\}$-vector of Hamming weight exactly $r$. For each such distinct coefficient vector, consider the vector $\bx = \tbx \circ \bz \circ -1$. By construction, it follows that ${\bf B}_{\rm int}\bx = (2{\bf B}\tbx - 2{\bf y}) \circ({\bf B}_{\rm BCH}{\bf z} - {\bf s})$ is a $\{0,1,2\}$-vector and $\|{\bf B}_{\rm int}\bx\|_p^p = 2^p\|{\bf B}\tbx - {\bf y}\|_p^p + \|{\bf B}_{\rm BCH}{\bf z} - {\bf s}\|_p^p\leqs 2^pt + r$. Since the number of such vectors is at least the number of distinct coefficient vectors $\mathbf{z}$, it can be lower bounded by
	\begin{equation*}
	\frac{1}{100} \cdot 2^{-h}{m \choose r} \geqs \frac{1}{100} \cdot 2^{-\frac{l}{2}\log m} {m \choose r} \geqs \frac{1}{100} \cdot \frac{m^r}{r^r m^{l/2}} \geqs \frac{1}{100} \cdot \frac{m^r}{l^l m^{l/2}}.
	\end{equation*}
	\noindent Finally, observe that each $\bz$ produces different $\bB_{\rm BCH}\bz$ and hence all $\bB_{\rm int}\bv$'s are distinct.
\end{proof}	
	
\begin{lemma}				\label{lem:annoying-vectors}
	Let $(\mathbf{B},\mathbf{y},t)$ be a NO instance, and let $\mathbf{B}_{\rm int}$ be the corresponding intermediate lattice. Then the number of annoying vectors for $\mathbf{B}_{\rm int}$ is at most $10^{-5}{m^{r}}\Big({100 m^{l/2}{l}^{l}}\Big)^{-1}$.
\end{lemma}

\begin{proof}
	Consider $\bx \in \mathbb{Z}^{q + m + h + 1}$ such that $\bB_{\rm int}\mathbf{x}$ is an annoying vector. We partition the vector and write it as $\bx = \bx_1 \circ \bx_2 \circ x$ where $\bx_1 \in \Z^q$, $\bx_2 \in \Z^{m + h}$ and $x \in \Z$. Using this, we can express $\bB_{\rm int}\bx$ as $\bB_{\rm int}\mathbf{x} = (2\bB\bx_1 - 2x\cdot\by)\circ(\bB_{\rm BCH}\bx_2 - x\cdot \mathbf{s})$.
	
	Suppose $x \neq 0$. Since $(\bB,\by,t)$ is a NO instance, the vector $[2\bB \enskip {\bf 0} \enskip 2\by]\cdot\bx = 2\bB\bx_1 - 2x\cdot\by$ has Hamming weight at least $l$. This would imply that $\bB_{\rm int}\bx$ cannot by annoying, which is a contradiction.  
	
	Thus, we henceforth can assume that $x = 0$; note that we now have $\bB_{\rm int}\mathbf{x} = (2\bB\bx_1) \circ (\bB_{\rm BCH}\bx_2)$. We further claim that, if $\bB_{\rm int}\mathbf{x}$ is annoying, then all of its coordinates must be odd. To see that this is the case, let us consider any $\bx$ such that $\bB_{\rm int}\bx$ has at least one odd coordinate. From $\bB_{\rm int}\mathbf{x} = (2\bB\bx_1) \circ (\bB_{\rm BCH}\bx_2)$, $\bB_{\rm BCH}\bx_2$ must have at least one odd coordinate. Let us further write $\bx_2$ as $\bx_2 = \bw_1 \circ \bw_2$ where $\bw_1 \in \Z^m$ and $\bw_2 \in \Z^h$. Notice that $\bB_{\rm BCH} \bx_2 = \bw_1 \circ (Q(\bP_{\rm BCH}\bw_1 - 2\bw_2))$. Since every coordinate of $\bB_{\rm BCH} \bx_2$ must be less than $Q$ in magnitude, it must be the case that $\bP_{\rm BCH}\bw_1 - 2\bw_2 = \vzero$. In other words, $(\bw_1 \mod 2)$ is a codeword of the BCH code. However, since the code has distance $l$, this means that, if $\bw_1$ has at least one odd coordinate, it must have at least $l$ odd (non-zero) coordinates. This contradicts to our assumption that $\bB_{\rm int}\mathbf{x}$ is annoying.
		 
	Therefore, $\bB_{\rm int}\bx$ must have less than $l/2^p$ non-zero coordinates, all of which are bounded in magnitude by ${l}^{10l}$. Hence, we can bound the total number of annoying vectors by
	\begin{eqnarray*}
	\big(2{l}^{10l} + 1\big)^{l/2^p}{{n + m + h}\choose {\lfloor \frac{l}{2^p} \rfloor}} \leqs (2l)^{10l^2} (n + m + h)^{l/2^p}
	\leqs (2l)^{10l^2} ((1 + l/2^p)m)^{l/2^p}
	\leqs e(2l)^{10l^2}m^{l/2^p}
	\end{eqnarray*}
\noindent where the second-to-last step holds since $h \leqs \frac{l}{2}\log m \leqs \frac{l m}{2^{p+1}}$ and $n \leqs \frac{m}{2^{p+1}}$. On the other hand,
	\begin{equation*}
	\frac{m^{r}}{m^{l/2}{l}^{l}} = \frac{m^{\big(\frac12 + \frac1\eta + \frac{1}{2^p}\big)l}}{m^{l/2}{l}^{l}} = m^{l/2^p} (m/l^\eta)^{l/\eta} \geqs m^{l/2^p} (100l)^{99l^2} \geqs 10^5 \left(e(2l)^{10l^2}m^{l/2^p}\right).
	\end{equation*}
\noindent which follows from our choice of $m$. Combining the bounds completes the proof.
\end{proof}

\subsection{The $\svp_{p,\gamma}$-instance}					\label{sec:final-lattice}

Finally, we construct $\bB_{\rm svp}$ from $\bB_{\rm int}$ by adding a random homogeneous constraint as in \cite{Khot05}. For ease of notation, let $N_g$ denote the lower bound on the number of distinct coefficient vectors guaranteed by Lemma \ref{lem:good-vectors} in the YES case. Similarly, let $N_a$ denote the upper bound on the number of annoying vectors as given in Lemma \ref{lem:annoying-vectors}. Combining the two Lemmas we have $N_g \geqs 10^5N_a$, which will be used crucially in the construction and analysis of the final lattice.
\paragraph{Construction of the Final Lattice}: Let $\rho$ be any prime number in{\footnote{Note that the density of primes in this range is at least $1/\log N_g = 1/r\log m$. Therefore, a random sample of size $O(r\log m)$ in this range contains a prime with high probability. Since we can test primality for any $\rho \in \Big[10^{-4}N_g, 10^{-2}N_g\Big]$ in FPT time, this gives us an FPT algorithm to sample such a prime number efficiently .}} $\Big[10^{-4}N_g, 10^{-2}N_g\Big]$. Furthermore, let ${\bf r} \overset{\rm unif}{\sim} [0,\rho-1]^{n + m + h}$ be a uniformly sampled lattice point. We construct ${\bf B}_{\rm svp}$ as 
\begin{align*}
	\bB_{\rm svp} =
	\begin{bmatrix}
		\bB_{\rm int} &  {0}  \\
		D\cdot{\bf r}\bB_{\rm int} &  D\cdot \rho 
	\end{bmatrix}
	\in \Z^{(n + m + h + 1) \times (q + m + h + 2)}.
\end{align*}

\noindent where $D = l^{10l}$. In other words, this can be thought of as adding a random linear constraint to the intermediate lattice. The choice of parameters ensures that with good probability, in the YES case, at least one of the good vectors ${\bf x} \in\mathbb{Z}^{q + m + h + 1}$ evaluates to $0$ modulo $\rho$ on the random constraint, and therefore we can pick $u \in \Z$ such that ${\bf B}_{\rm svp}({{\bf x} \circ u}) = (\bB_{\rm int}\bx) \circ 0$ still has small $\ell_p$ norm. On the other hand, since $N_a \ll N _g$, with good probability, all of annoying vectors evaluate to non-zeros, and hence will contribute a coordinate of magnitude $D = l^{10l}$. This intuition is formalized below.

\begin{lemma}					\label{lem:svp-lattice}
	Let $(\bB,\by,t)$ be a $\snvp_{p,\eta}$ instance as given by Lemma \ref{lem:csp-to-snvp}, and let $\bB_{\rm svp} \in \mathbb{Z}^{(n + m + h + 1)\times(q + m + h + 2)}$ be the corresponding final lattice. Then the following conditions hold:
	\begin{itemize}
		\item If $(\bB,\by,t)$ is an YES instance, then w.p. $0.8$, there is $\mathbf{x} \in \mathbb{Z}^{q + m + h + 2}$ such that $ \|\bB_{\rm svp}\bx\|^{p}_p \leqs \gamma^{-1}_p\eta t$.
		\item If $(\bB,\by,t)$ is a NO instance, then w.p. $0.9$, $\bB_{\rm svp}\mathbf{x}$ is not annoying for every $\bx \in \Z^{q + m + h + 2}$. In particular,  we have $\|\bB_{\rm svp}\bx\|^p_p \geqs \eta t$.
	\end{itemize}
	Here $\gamma^{-1}_p := \frac12 + (2^p+1)/\eta + 1/2^p$ is strictly less than $1$ by our choice of $\eta$. 
\end{lemma}
\begin{proof}
	Let $(\bB,\by,t)$ be a NO instance and fix a vector ${\bf x}\circ u \in \Z^{q + m + h + 2}$. If $\bx$ is not an annoying vector w.r.t. the intermediate lattice $\bB_{\rm int}$, then it follows that $\bx\circ u$ is also not an annoying vector w.r.t. the final lattice $\bB_{\rm svp}$. Therefore, it suffices to look at vectors $\bx \circ u$ such that $\bx$ is annoying w.r.t. $\bB_{\rm int}$. By construction, $(\bB_{\rm svp}(\bx \circ u))_{(n + m + h + 1)} = 0$ implies that $ {\bf r}\bB_{\rm int}\bx = u\cdot \rho$, which in turn is equivalent to ${\bf r}\bB_{\rm int}\bx \equiv 0 \mod \rho$. Since, $\bx_i < \rho$ for every $i \in [q + m + h + 1]$, this event happens with probability exactly $1/\rho$ over the random choice of $\mathbf{r}$ (for any arbitrary $u \in \mathbb{Z}$). Therefore by union bound, for every choice of annoying vector $\bx$ and coefficient $u$, we have ${\bf r}\bB_{\rm int}\bx \neq u\cdot \rho$, with probability at least $1 - N_a/\rho \geqs 0.9$. And therefore, with probability at least $0.9$, for every annoying $\bx$, the last coordinate of $\bB_{\rm svp}(\bx \circ u)$ has magnitude at least $D$.
	
	Next, let $(\bB,\by,t)$ be an YES instance. We condition on the event that there exists at least $N_g$ good vectors as guaranteed by Lemma \ref{lem:good-vectors}. Consider any two distinct vectors $\bx_1,\bx_2 \in \Z^{q + m + h + 1}$ provided by Lemma \ref{lem:good-vectors}. Since $\bB_{\rm int}\bx_1$ and $\bB_{\rm int}\bx_2$ are distinct $\{0, 1, 2\}$-vectors, they are pairwise independent modulo $\rho > 2$. Therefore, instantiating Lemma 5.8 from \cite{Khot05} with the lower bound on the number of good vectors $N_g$, and our choice of $\rho$, it follows that with probability at least $0.9$, there exists a good vector ${\bf x}$ such that ${\bf r}\bB_{\rm int}\bx \equiv 0 \mod \rho$. Therefore, by union bound, with probability at least $0.8$ (over the randomness of Lemma \ref{lem:good-vectors} and the choice of $\mathbf{r},\rho$), there exists $\bx$ such that, for some $u \in \Z$, $\|\bB_{\rm svp}(\bx \circ u)\|_p^p = \|\bB_{\rm int}\bx\|_p^p \leqs 2^p t + r = \gamma_p^{-1}l$, which concludes the proof.
\end{proof}

Finally, observe that given the $\snvp_{p,\eta}$-instance $(\bB,\by,t)$, we can construct $\bB_{\rm svp}$ in $t^{O(t)}\cdot{\rm poly}(n,q)$-time. This, along with guarantees of Lemma~\ref{lem:svp-lattice}, completes the proof of Lemma \ref{lem:snvp-to-svp}. 

\subsection{Gap Amplification for $\svp_{p,\gamma}$}	\label{sec:svp-gap-amp}

As in the case of $\mdp$, we use tensor product of lattices to boost the hardness of $\svp$ to any constant factor. The tensor product of lattices is defined similarly as in the case of linear codes. Given $\bA \in \Z^{m \times m'}$, let $\mathcal{L}(\bA)$ be the lattice generated by $\bA$. Given matrices $\bA \in \Z^{m \times m'}$ and $\bB \in \Z^{n \times n'}$ the tensor product of $\mathcal{L}(\bf A)$ and $\mathcal{L}(\bB)$ is defined as 
\begin{equation}
\mathcal{L}(\bA) \otimes \mathcal{L}(\bB) = \{ \bA\mathbf{X}\bB^\top | \mathbf{X} \in \Z^{m' \times n'}\}
\end{equation}
For brevity, let $\mathcal{L}_1 = \mathcal{L}(\bf A)$ and $\mathcal{L}_2 = \mathcal{L}(\bB)$. Furthermore, for any lattice $\mathcal{L}$, and $p \geqs 1$, let $\lambda_p(\mathcal{L})$ be the length of the shortest vector in the $\ell_p$ norm. We first show how the tensor product for $\svp_{2,\gamma}$, and then show how to modify the arguments to show gap amplification for arbitrary $p$. The following lemma from \cite{HR07} summarizes the properties of tensor product instances of $\svp_{2,\gamma}$.

\begin{lemma}				\label{lem:lattice-gap-amp}
	Let $\mathcal{L}_1$ and $\mathcal{L}_2$ be as above. Then for any $p \geqs 1$ we have $\lambda_2(\mathcal{L}_1 \otimes \mathcal{L}_2) \leqs \lambda_2(\mathcal{L}_1)\cdot\lambda_2 (\mathcal{L}_2)$. Furthermore, suppose every vector $\by \in \mathcal{L}_1$ satisfies at least one of the following conditions:
	\begin{itemize}
		\item The vector $\by$ has Hamming weight at least $l$.
		\item The vector $\by$ is even and has Hamming weight at least $l/4$.
		\item The vector $\by$ is even and $\|\by\|_\infty \geqs D$
	\end{itemize}
	where $D = l$. Then, $\lambda_2(\mathcal{L}_1 \otimes \mathcal{L}_2) \geqs l^{1/2}\cdot\lambda_2(\mathcal{L}_2)$
\end{lemma}

It is easy to see that given a $\svp_{2,\gamma}$ instance $(\bA,k)$ (as in Lemma \ref{lem:snvp-to-svp}), the tensor product gives an FPT reduction to $\svp_{2,\gamma^2}$. Indeed, if $(\bA,k)$ is a YES instance, then $\lambda_2(\mathcal{L}(\bA) \otimes \mathcal{L}(\bA))^2 \leqs k^2$. Conversely, if $(\bA, k)$ is a NO instance, then setting $l = \gamma \cdot k$ in Lemma \ref{lem:lattice-gap-amp}, we get $\lambda_2(\mathcal{L}(\bA)  \otimes \mathcal{L}(\bA))^p \geqs l^2 = \gamma^2k^2$. Therefore, by repeated tensoring, the FPT gap hardness can be amplified to any constant. We now give a sketch of proof of Lemma \ref{lem:lattice-gap-amp}, which will be needed to illustrate modifications to the proof required to show gap amplification for $p \neq 2$.


\begin{proof}[Proof Sketch of Lemma \ref{lem:lattice-gap-amp}]
	The first part of the statement is well known for every $p \ge 1$, so we shall only prove the lower bound. Fix a $\bv \in \mathcal{L}_1 \otimes \mathcal{L}_2$, and let $l = \lambda_2(\mathcal{L}_1)^2$. Then using a change of basis argument, we can write $\bv = \bU\bW^\top = \sum_{i \in [r]} \mathbf{u}_i\mathbf{w}^\top_i$ such that (i) $\bU$ and $\bW$ are full column rank matrices (ii) The vectors $\{\mathbf{u}_1,\mathbf{u}_2,\ldots,\mathbf{u}_r\}$ belong to $\mathcal{L}_1$, and (iii) The vectors $\{\mathbf{w}_1,\mathbf{w}_2,\ldots,\mathbf{w}_r\}$ belong to $\mathcal{L}_2$. Let $\mathcal{L}' = \mathcal{L}(\bU)$ be the lattice generated by the columns of $\bU$. By construction, it follows that $\mathcal{L}' \subset \mathcal{L}_1$. Therefore invoking Claim 3.5 from \cite{HR07}, we know that at least one of the following conditions hold:
	\begin{itemize}
		\item[1.] The matrix $\bU$ has at least $l$ non-zero rows.
		\item[2.] The matrix $\bU$ is even and has at least $l/4$ non-zero rows.
		\item[3.] ${\rm det}(\mathcal{L}') \ge D^{r/2}  =l^{r/2}$.
	\end{itemize}
	
	We analyze each of the above cases individually:
	
	\noindent{\bf Case 1}: Since $\bU$ has at least $l$ non-zero rows, and $\bW$ has full column rank, $\bv = \bU\bW^\top$ also has at least $l$ non-zero rows. Furthermore, each row of $\bv$ belongs to $\mathcal{L}'$, and therefore, each non-zero row has $\ell_2$ norm at least $\lambda_2(\mathcal{L}_2)$. Therefore, $\|\bv\|_2 \ge \sqrt{l}\cdot\lambda_2(\mathcal{L}_2)$.
	
	\noindent{\bf Case 2}: Since $\bU$ has at least $l/4$ non-zero rows and is even, $\bv = \bU\bW^\top$ is even and has at least $l/4$ non-zero rows. Using arguments as above, we again have $\|\bv\| \ge \sqrt{l/4}\cdot.2\lambda_2(\mathcal{L}_2) \ge \sqrt{l}\cdot\lambda_2(\mathcal{L}_2).$
	
	\noindent{\bf Case 3}: Here we have ${\rm det}(\mathcal{L}({\bU})) \ge l^{r/2}$. The key step used in this case is the following inequality (Claim 3.6~\cite{HR07}), which can be used to lower bound $\|\bv\|_2$ as 
	\begin{equation}			\label{eq:det-bound}
	\|{\bv}\|_2 \ge \sqrt{r}\Big({\rm det}(\mathcal{L}(\bU){\rm det}(\mathcal{L}(\bW)\Big))^{1/r}
	\end{equation} 
	
	Now ${\rm det}(\mathcal{L}(\bU)) \ge l^{r/2}$, and using \emph{Minkowski's Theorem} \cite{MG12}, we get the lower bound ${\rm det}(\mathcal{L}(\bW)) \ge \Big(\lambda_2(\mathcal{L}(\bW))/\sqrt{r}\Big)^{1/r}$. Plugging in these bounds in \eqref{eq:det-bound} gives us $\|\bv\|_2 \ge \sqrt{l}\lambda_2(\mathcal{L}(\bW))	\ge \sqrt{l}\lambda_2(\mathcal{L}_2)$.
\end{proof}	
	

\paragraph{Gap Amplification for $p \neq 2$}

Towards generalizing the proof of Lemma \ref{lem:lattice-gap-amp} to any $p \in [1,\infty)$, it is easy to see that Cases 1 and 2 of the proof hold as is, when $\mathcal{L}_1$ is the corresponding $\ell_p$ variant of the hard instance from Theorem \ref{thm:SVPmain}. For Case 3, the obstacle is that the lower bound from \eqref{eq:det-bound} is known only for the $\ell_2$ norm. However, this can be handled by using the relationship between the counting norms i.e., if $\bv$ is a $T$-length vector, then $\|\bv\|_p \ge T^{1/p - 1/2}\|\bv\|_2$ for all $p \ge 2$, and $\|\bv\|_p \ge \|\bv\|_2$ for all $p \in [1,2]$. Fix a $p >2$ (the case $p \in (1,2)$ is simpler). Suppose for $\mathcal{L}'$ we have the following stronger guarantee ${\rm det}(\mathcal{L}') \ge (T^2l)^{r}$ (which can be achieved by choosing the parameters $D,Q$ to be dependent on $T$ in the proof of Lemma \ref{lem:snvp-to-svp}). Then using \eqref{eq:det-bound} and the $\ell_p$ variant of Minkowski's Theorem we get 
\begin{eqnarray*}
\|\bv\|_p \ge T^{1/2-1/p}\|\bv\|_2 &\ge& T^{1/2 - 1/P} \cdot \sqrt{r}\Big({\rm det}(\mathcal{L}'){\rm det}(\mathcal{L}(\bW))\Big)^{1/r}\\
&\ge& T^{1/2 - 1/P}  \sqrt{r}\Big(T^{2r}l^{r}\Big)^{1/r}\bigg(\frac{\lambda_p(\mathcal{L}(\bB))}{r^{1/p}}\bigg)\\
 &\ge& l^{1/p}\lambda_p(\mathcal{L}(\bB)).
\end{eqnarray*}

Therefore, the proof of Lemma \ref{lem:lattice-gap-amp} can be extended (for any fixed $p$) whenever $\svp_{p,\gamma_p}$ instances have stronger guarantees in the NO case. In particular, following strengthened version of Lemma \ref{lem:snvp-to-svp} suffices, which can be shown using identical arguments.

\begin{lemma}				\label{lem:snvp-to-svp-strong}
	Fix  constants $p > 1$, $c \in \N$, and let $\eta \geqs 1$ be such that $\frac12 + \frac{1}{2^p} + \frac{(2^p + 1)}{\eta} < 1$. Let $(\bB,\by,t)$ be a $\snvp_{p,\eta}$ instance, as given by Lemma \ref{lem:csp-to-snvp}. Then, for some constant $\gamma_p > 1$, there is a randomized FPT reduction from $\snvp_{p,\eta}$ instance $(\bB,\by,t)$ to $\svp_{p,\gamma}$ instance $(\bB_{\rm svp},\gamma^{-1}_pl)$ (where $\bB_{\rm svp} \in \Z^{n_1 \times q_1}$) with $l = \eta \cdot t$ with the following properties. 
	
	(YES): If $(\bB,\by,t)$ is a YES instance, then w.p. $0.8$, there exists $\bx$ such that $\|\bB_{\rm svp}\bx\|^p_p \leqs \gamma^{-1}_p l$. 
	
	(NO): If $(\bB,\by,t)$ is a NO instance then w.p. at least $0.8$, for all choices of $\bx$, the vector $\bB_{\rm svp}\bx$ satisfies at least one of the following conditions:
	\begin{itemize}
		\item[1.] The Hamming weight of $\bB_{\rm svp}\bx$ at least $l$.
		\item[2.] All coordinates of $\bB_{\rm svp}\bx$ are even, and its Hamming weight is at least $l/2^p$.
		\item[3.] All coordinates of $\bB_{\rm svp}\bx$ are even, and it has at least one coordinate of magnitude at least $D = {n_1}^{100c}\cdot l$. 
	\end{itemize}	
	In particular, every vector $\bB_{\rm svp}\bx$ satisfies $\|\bB_{\rm svp}\bx\|^p_p \ge l$.
\end{lemma}

Additionally, by modifying Case 3 in the proof of Lemma \ref{lem:lattice-gap-amp} via the equivalence of norms argument, we can prove the following variant:

\begin{lemma}				\label{lem:lattice-gap-amp-strong}
	Fix $p > 1$, $c \in \N$, and let $(\bB_{\rm svp},k)$ be a $\svp_{p,\gamma_p}$ instance (where $\bB_{\rm svp} \in \Z^{n_1 \times q_1}$) as given by Lemma \ref{lem:snvp-to-svp-strong} for the given choice of parameters $c,p$. Consider any lattice $\mathcal{L}_2 \in Z^{n^{i}_1}$, where $i \le n$. Then $\lambda_p(\mathcal{L}(\bB_{\rm svp}) \otimes \mathcal{L}_{2}) \ge \lambda_p(\mathcal{L}(\bB_{\rm svp}))\cdot\lambda_p(\mathcal{L}_2)$.
\end{lemma}

Now, fix any $p > 1$. Suppose we want to boost the gap from $\gamma_p$ (as given by Lemma \ref{lem:snvp-to-svp-strong}) to $(\gamma_p)^{c'}$ for some $c' \in \N$. We instantiate Lemma \ref{lem:snvp-to-svp-strong} with $c = c'$, and let $(\bB_{\rm svp},k)$ be the corresponding $\svp_{p,\gamma_p}$ instance. Let $\mathcal{L}_1 = \mathcal{L}(\bB_{\rm svp})$ be the lattice generated by it. For $i \le c'$, we construct the tensored instances $\mathcal{L}_i = \mathcal{L}_1 \otimes \mathcal{L}_{i-1}$. 

Fix such an $i \in [c']$. If $(\bB_{\rm svp},k)$ is a YES instance, then using Lemma \ref{lem:lattice-gap-amp} we get $\lambda_p(\mathcal{L}_i)^p \le k \cdot \lambda_p(\mathcal{L}_{i-1})^p$, which recursively implies that $\lambda_p(\mathcal{L}_i)^p \le k^{i}$. Conversely, let $(\bB_{\rm svp},k)$ be a NO instance. By construction, it follows that $\mathcal{L}_i \subseteq \Z^{n^{i}}$, where $i \le c'$. Using Lemma \ref{lem:lattice-gap-amp-strong} we get $\lambda_p(\mathcal{L}_i)^p \ge (\gamma_pk) \lambda_p(\mathcal{L}_{i-1})^{p}$, which again by recursion implies $ \lambda_p(\mathcal{L}_i)^p \ge (\gamma_pk)^i$. Since these conditions hold for every $i \in [c']$, this gives us an FPT reduction from $\svp_{p,\gamma_p}$ to $\svp_{p,\gamma^{c'}_p}$.



